Beyond Triplet: Leveraging the Most Data for Multimodal Machine Translation

Multimodal machine translation (MMT) aims to improve translation quality by incorporating information from other modalities, such as vision. Previous MMT systems mainly focus on better access and use of visual information and tend to validate their methods on image-related datasets. These studies face two challenges. First, they can only utilize triple data (bilingual texts with images), which is scarce; second, current benchmarks are relatively restricted and do not correspond to realistic scenarios. Therefore, this paper correspondingly establishes new methods and new datasets for MMT. First, we propose a framework 2/3-Triplet with two new approaches to enhance MMT by utilizing large-scale non-triple data: monolingual image-text data and parallel text-only data. Second, we construct an English-Chinese {e}-commercial {m}ulti{m}odal {t}ranslation dataset (including training and testing), named EMMT, where its test set is carefully selected as some words are ambiguous and shall be translated mistakenly without the help of images. Experiments show that our method is more suitable for real-world scenarios and can significantly improve translation performance by using more non-triple data. In addition, our model also rivals various SOTA models in conventional multimodal translation benchmarks.

==> 030formulation.tex <==
% Given an image $i$ and their associated text in source language $x$ , the multimodal machine translation aims to translate the text  $x$ to the target language  $y$ with the enhanced information from the image. 

% Conventional multimodal MT systems focus on training on triple dataset, where each sample is consists of a image,  its describing sentence in source language and the translated sentence in target language. The conventional models requires both training and testing sets in a triple form $\{(x, y, i)\}$. 

% However, the well-labelled triples  $(x, y, i)$ are expensive, scarce and difficult to obtain. Considering that training big models via massive data has orientated the academic frontier and industrial practice, conventional systems become less prominent on real-world applications since their approaches are valid only on the insufficient datasets. On the other hand, the bilingual parallel corpus without images and the image-text pairs of the target language are then easily accessible, which have large potential to enhance multimodal translation models.

% Therefore, we reformulate the multimodal machine translation to make it more relevant for realistic scenarios. Given the adequate parallel corpus $\{ (x, y) \}$, image caption pairs in target language $\{ (i, y) \} $ and a small multimodal triple set $\{(x, y, i)\}$. 
% %\shanbo{theoretically we also have $\{ (x, i) \}$? but we did not use though} 有使用，但也可以不用，我写作改一下
% Our task is to construct a multimodal translation system based on this data. 
% The constructed system shall give an accurate translation $y$ for any given new sentence $x$ and its corresponding image $i$. 

% In real world scenarios, the multimodal triples can be absent. Hence we hope the model only utilize bilingual and caption data for training while can still inference on multimodal input, we refer this setting as zero-shot triples in the Experiments. 


==> tables/ablation.tex <==
\begin{table}[h]
\centering
\resizebox{.5\textwidth}{!}{
\begin{tabular}{l|l|ll}
\hline
id &                       & test         & dev          \\ \hline
19 & soft-fusion-adversial & 40.49(+2.67) & 54.72(+1.34) \\
20 & soft-fusion-absent    & 37.85(+0.03) & 53.32(-0.06) \\
21 & hard-fusion-adversial & 36.95(-0.87) & 53.23(-0.15) \\
22 & hard-fusion-absent    & 38.32(+0.50)  & 54.02(+0.64) \\ \hline
\end{tabular}

}
\label{tab:ablation}
\caption{BLEU score on vision ablation study. We indicate the BLEU change compared with plain Transformer~(\ie row 12 in Table~\ref{tab:main})  (TODO to bar chart)}
\end{table}

==> tables/cases.spare.tex <==
\begin{table*}[h]
% 	\renewcommand{\arraystretch}{1.0}
	\centering
	\resizebox{.83\textwidth}{!}
	{%
	\begin{tabular}{cll@{}}
	\toprule
	\MR{8}{*} {\includegraphics[height=2.1cm]{figs/case_holder.jpeg}} 
	& \T{source:} & winnie the pooh table organizers stationeries holder \\
	& \T{human:} &  小熊\ 维尼\ 桌面\ 整理\ 器\ 文具\ 架 \\
	& \T{Plain:} &  \sout{winnie}\ 维尼\ \underline{桌}\ \sout{组织}\ \  文具\  \underline{支架} \\
	& \phantom{\T{ Plain:}} &  \sout{winnie} winnie \underline{table} \sout{organize} stationery \underline{bracket} \\
% 	& \T{Plain:} &  \sout{12 }\ \ 维尼\ 桌\ \ {组织}\ \  文具\ \ {支架}\ \\
% 	& \phantom{\T{ Plain:}} &  {winnie} winnie {table} {organize} stationery \underline{bracket} \\
	& \T{Ours (Triplet-only):}  & 维尼\  \underline{桌子}\  \textbf{收纳}\  文具\  \underline{盒} \\
	& \phantom{\T{\method:}} &  winnie \underline{table} \textbf{organizers} stationery \underline{box}  \\
	& \T{Ours (All-data):} &  \textbf{维尼}\  \textbf{熊}\  \textbf{桌面}\  \textbf{收纳}\  盒\  文具\  \textbf{收纳}\  架 \\
	& \phantom{\T{\methodext:}} &  \textbf{bear winnie} \textbf{desk} \textbf{organizer} box stationery \textbf{organizer} holder \\

    \midrule
	\MR{8}{*} {\includegraphics[height=2.1cm]{figs/case_mask.jpeg}} 
	& \T{source:} & ready stock kids medical surgical face mask 3-ply 20pcs \\
	& \T{human:} &  现货\ 儿童\ 医疗\ 手术\ 口罩\ 3\ 层\ 20\ 个 \\
	& \T{Plain:} &  现货\ 儿童\ 医用\ \sout{面具}\ 3\sout{-ply}\ 20\sout{pcs}\ \\
	& \phantom{\T{ Plain:}} &  ready stock kids medical \sout{(opera) mask} 3-\sout{ply} 20\sout{pcs}\\
	& \T{Ours (Triplet-only):}  & 现货\ 儿童\ 医用\ \textbf{口罩}\ 3\sout{ply}\ 20\sout{pcs}\ \\
	& \phantom{\T{\method:}} &  ready stock kids medical \textbf{mask} 3-\sout{ply} 20\sout{pcs}  \\
	& \T{Ours (All-data):} &  现货\ 儿童\ 医用\ 外科\ \textbf{口罩}\ 3\ \textbf{层}\ 20\ \textbf{片}\ \\
	& \phantom{\T{\methodext:}} &  ready stock kids medical surgical \textbf{mask} 3-\textbf{ply} 20\textbf{pcs} \\
	
	\bottomrule
	\end{tabular}
	}
	\caption{Qualitative examples from two complex scenarios. Plain and Ours (Triplet-only) respectively indicate plain Transformer and \method trained on triple data only, and  Ours (All-data) indicate \method trained on all data.  The \sout{strikethrough},  \underline{underline} and \textbf{bold}  indicates inappropriate, reluctant and excellent choices respectively. 
	The more detailed comments on the translation are in Appendix. }
	\label{tab:case_study}
\end{table*}

==> tables/main.tex <==
\begin{table}[]
\begin{tabular}{l|lll}
\hline
ID & \multicolumn{1}{l|}{}                     & test     & dev     \\ \hline
1  & \multicolumn{1}{l|}{Transformer}          & 33.21    & 48.83   \\
2  & \multicolumn{1}{l|}{SA+GF+ViT}            & 33.46    & 49.22   \\
3  & \multicolumn{1}{l|}{SA+GF+CLIP}           & 33.07    & 48.27   \\
4  & \multicolumn{1}{l|}{UVR-NMT}              & 32.23    & 47.77   \\
5  & \multicolumn{1}{l|}{soft-fusion}          & 37.18    & 49.4    \\
6  & \multicolumn{1}{l|}{hard-fusion}          & 37.2     & 49.92   \\
7  & \multicolumn{1}{l|}{soft+hard-fusion}     & 36.96    & 49.32   \\ \hline
   & \multicolumn{3}{c}{+Bilingual translation}                     \\ \hline
8  & \multicolumn{1}{l|}{plain Transformer}    & 35.23    & 50.82   \\
9  & \multicolumn{1}{l|}{soft-fusion}          & 39.63    & 52.92   \\
10 & \multicolumn{1}{l|}{hard-fusion}          & 38.22    & 52.29   \\
11 & \multicolumn{1}{l|}{soft+hard-fusion}     & 39.36    & 52.52   \\ \hline
   & \multicolumn{3}{c}{+Bilingual translation+Monolingual Caption} \\ \hline
12 & \multicolumn{1}{l|}{plain Transformer}    & 37.82    & 53.38   \\
13 & \multicolumn{1}{l|}{soft-fusion}          & 41.49    & 55.47   \\
14 & \multicolumn{1}{l|}{hard-fusion}          & 40.79    & 54.77   \\
15 & \multicolumn{1}{l|}{soft+hard-fusion}     & 41.18    & 54.92   \\ \hline
   & \multicolumn{3}{c}{Zero-shot  Triple Data}                     \\ \hline
16 & \multicolumn{1}{l|}{soft-fusion}          & 39.72    & 54.36   \\
17 & \multicolumn{1}{l|}{hard-fusion}          & 39.68    & 53.78   \\
18 & \multicolumn{1}{l|}{soft+hard-fusion}     & 40.17    & 53.87   \\ \hline
\end{tabular}
\caption{(TODO)BLEU score on \data }
\label{tab:main}
\end{table}




==> tables/main2.tex <==






\begin{table*}[]
\centering
\begin{tabular}{c|l|cccccc}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{ID} & \multirow{2}{*}{Model and Variants}     & \multicolumn{2}{c|}{Triplet Only}                           & \multicolumn{2}{c|}{+ PT}        & \multicolumn{2}{c}{+ PT + MC}  \\  \cline{3-8}
& & Test                 & \multicolumn{1}{c|}{Dev}            & Test                      & \multicolumn{1}{c|}{Dev}            & Test                 & Dev                  \\ \hline
1  & Plain Transformer              & 34.21                & \multicolumn{1}{c|}{48.89}          & 35.51                     & \multicolumn{1}{c|}{53.42}          & 37.82                & 53.38                \\
2  & Selective Attention      & 36.39                & \multicolumn{1}{c|}{48.05}          & /                         & \multicolumn{1}{c|}{/}              & /                    & /                    \\
3  & UPOC$^2$ & 35.06                   &  \multicolumn{1}{c|}{48.66}             & /                         & \multicolumn{1}{c|}{/}              & /                    & /                    \\
4                                                                                                 & UVR-NMT                                 & 32.23                           & \multicolumn{1}{c|}{47.77} & 36.88                           & \multicolumn{1}{c|}{52.80} & /                               & /                               \\ \hline

5  & \soft              & 37.18                & \multicolumn{1}{c|}{49.40}          & 39.63                     & \multicolumn{1}{c|}{52.92}          & 41.49                & \textbf{55.47}                \\
6  & \hard              & \textbf{37.20}       & \multicolumn{1}{c|}{\textbf{49.92}} & 38.22                     & \multicolumn{1}{c|}{52.29}          & 40.79                & 54.77                \\
7  & \textsc{Fusion+Prompt}         & 37.03                & \multicolumn{1}{c|}{49.42}          & \textbf{40.10}            & \multicolumn{1}{c|}{\textbf{53.77}} & \textbf{41.62}       & 54.92       \\ \hline
   & Google Translate         & \multicolumn{1}{l}{}            & \multicolumn{2}{c}{39.41} & \multicolumn{2}{c}{58.49}           & \multicolumn{1}{l}{} \\ \Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results of \method and related work on \data. ``PT'' indicates parallel text data $\{(x, y)\}$, ``MC'' indicates monolingual caption data $\{(y, i)\}$. On the one hand, \method outperforms previous studies. On the other hand, extra non-triple data brings significant improvements. Note that the dev set and training set have the same distribution, and only the test set consists of carefully selected samples that require images for translation, resulting in a larger difference in performance on Google Translate. }
\label{tab:main}
\end{table*}


==> tables/main3.tex <==
\begin{table*}[]
\centering
\begin{threeparttable}[b]
\begin{tabular}{c|l|ccc|cc}
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{ID} & Test sets  & \multicolumn{3}{c|}{\data-test}                               & Multi30K-16       & Multi30K-17      \\ \cline{2-7} 
   & Training Data       & Triplet Only   & + PT                  & + PT + MC      & \multicolumn{2}{c}{Multi30K Triplet} \\ \hline
1  & Plain Transformer   & 34.21          & 35.51                 & 37.82          & 39.97             & 31.87            \\
2  & Selective Attention \tnote{$\spadesuit$} & 36.39          & /                     & /              & 40.63             & 33.80            \\
3  & UPOC$^2$    \tnote{$\diamondsuit$}          & 35.06          & /                     & /              & 40.8              & 34.1             \\ \hline
4  & UVR-NMT   \tnote{$\clubsuit$}           & 32.23          & 36.88                 & /              & 38.19             & 31.85            \\
5  & Phrase Retrieval\tnote{$\clubsuit$}     & /              & / & /              & 40.30             & 33.45            \\ \hline
6  & \soft                & 37.18          & 39.63                 & 41.49          & \textbf{40.95}    & 34.03            \\
7  & \hard                & \textbf{37.20} & 38.22                 & 40.79          & 40.17             & 33.87            \\
8  & \textsc{Fusion+Prompt}                 & 37.03          & \textbf{40.10}        & \textbf{41.62} & 40.48             & \textbf{34.62}   \\ \hline
   & Google Translate    & \multicolumn{3}{c|}{39.41}                              & 41.9              & 42.0             \\ \Xhline{3\arrayrulewidth}
\end{tabular}

 \begin{tablenotes}
 \scriptsize
 \item [$\clubsuit$] Multi30K's results copy from ~\citet{FangF22}. Phrase Retrieval is not reported on \data since they haven't released the phrase extraction scripts.
 \item [$\diamondsuit$] Multi30K's results copy from ~\citet{0003CJLXH21}. 
   \item [$\spadesuit$] We use their open source code to reproduce Multi30K's results.
 \end{tablenotes}

\caption{Results of \method and related work on \data. ``PT'' indicates parallel text data $\{(x, y)\}$, ``MC'' indicates monolingual caption data $\{(y, i)\}$. On the one hand, \method outperforms previous studies. On the other hand, extra non-triple data brings significant improvements. Our reported improvement is examied with \citet{ReichartDBS18}'s significance test with $p<0.05$~.
}
\label{tab:main}
\end{threeparttable}
\end{table*}

==> tables/multi30k.tex <==
\begin{table}[]
\begin{threeparttable}[b]
\begin{tabular}{c|l|cc}
\Xhline{3\arrayrulewidth}
ID   &        Models              & Test2016 & Test2017 \\ \hline
1  & Plain Transformer          & 39.97    & 31.87    \\ \hline
2  & UVR-NMT\tnote{$\clubsuit$}        & 38.19    & 31.85    \\
3  & Phrase Retrieval\tnote{$\clubsuit$}     & 40.30     & 33.45    \\
4  & UPOC$^2$\tnote{$\diamondsuit$}                & 40.8     & 34.1     \\
5  & Selective Attention\tnote{$\spadesuit$}
 & 40.63       & 33.80       \\ \hline
%  & selective attention  & 41.84    & 34.32    \\ \hline
6  & \soft          & \textbf{40.95}    & 34.03    \\
7  & \hard          & 40.17    & 33.87    \\
8 & \textsc{Fusion+Prompt}     &  40.48        &  \textbf{34.62}       \\ \hline
\  & Google Translate     & 41.9   & 42.0       \\  
\Xhline{3\arrayrulewidth}
\end{tabular}

 \begin{tablenotes}
 \scriptsize
 \item [$\clubsuit$] results copy from ~\citet{FangF22}
 \item [$\diamondsuit$] results copy from ~\citet{0003CJLXH21}
   \item [$\spadesuit$] 
%   Models' and baselines' results of the original paper were generally 2 BLEU higher than peer papers, where we think the difference comes from the BLEU measurement. 
   We use their open source code to reproduce.
%   and evaluate it with uniform BLEU script
 \end{tablenotes}


\caption{Results of \method and related work on Multi30K. }
\label{Tab:m30k}
\end{threeparttable}
\end{table}


% \footnote{Models' and baselines' results of the original paper were generally 2 BLEU higher than peer papers, where we think the difference comes from the BLEU measurement. We use their open source code to reproduce and evaluate it with uniform BLEU script}
